Division by four

Write A<=B if there is an injection from A to B, and A==B if there is a bijection. We give a simple proof that for finite n, nA<=nB implies A<=B. From the Cantor-Bernstein theorem it then follows that nA==nB implies A==B. These results have a long and tangled history, of which this paper is meant to be the culmination.

==> four_dot_bib <==
@book{hinkis,
author="Arie Hinkis",
title="Proofs of the Cantor-Bernstein Theorem: A Mathematical Excursion",
year="2013",
publisher="Birkhauser"
}


@article{schwartz:four,
title={{P}an {G}alactic {D}ivision},
author = {Rich Schwartz},
year="to appear",
journal={Mathematical Intelligencer},
xxxeprint={arXiv:math/XXXXXXX [math.LO]},
xxxnote={\url{http://arxiv.org/abs/math/XXXXXXX}},
}

@misc{conwaydoyle:three,
title={Division by three},
author = {Peter G. Doyle and John Horton Conway},
year="1994",
eprint={arXiv:math/0605779 [math.LO]},
note={\url{http://arxiv.org/abs/math/0605779}},
}

@misc{doyleqiu:four,
title={Division by four},
author = {Peter G. Doyle and Cecil Qiu},
year="2015",
eprint={arXiv:math/XXXXXXX [math.LO]},
note={\url{http://arxiv.org/abs/math/XXXXXXX}},
}

@book{bachmann:transfinite,
	author =	"H. Bachmann",
	title =		"Transfinite Zahlen (Zweite Auflage)",
	publisher =	"Springer",
	address =	"Berlin",
	year =		"1967"
}
@article{bernstein:mengenlehre,
	author =	"F. Bernstein",
	title =		"Untersuchungen aus der {M}engenlehre",
	journal =	"Math. Ann.",
	volume =	"61",
	year =		"1905",
	pages =		"117-154"
}
@article{garsiaMilne:rogers,
	author =	"A. M. Garsia and S. C. Milne",
	title =		"A {R}ogers-{R}amanujan bijection",
	journal =	"J. Combin. Theory, Series A",
	volume =	"31",
	year =		"1981",
	pages =		"289-339"
}
@book{jech:setTheory,
	author =	"T. Jech",
	title =		"Set Theory",
	publisher =	"Academic Press",
	address =	"New York",
	year =		"1978"
}

@article{lindenbaumTarski:ensembles,
	author =	"A. Lindenbaum and A. Tarski",
	title =		"Communication sur les recherches de la th\'{e}orie des ensembles",
	journal =	"Comptes Rendus des s\'{e}ances de la Soci\'{e}t\'{e} des Sciences et des Letters de Varsovie, Classe {I}{I}{I}",
	volume =	"19",
	year =		"1926",
	pages =		"299-330"
}

@book{nelson:predicative,
	author =	"E. Nelson",
	title =		"Predicative Arithmetic",
	publisher =	"Princeton University Press",
	address =	"Princeton",
	year =		"1986"
}

@article{remmel:partition,
	author =	"J. B. Remmel",
	title =		"Bijective proofs of some classical partition identities",
	journal =	"J. Combin. Theory, Series A",
	volume =	"33",
	year =		"1982",
	pages =		"273-286"
}

@article{sierpinski:two,
	author =	"W. Sierpinski",
	title =		"Sur l'\'{e}galit\'{e} $2m=2n$ pour les nombres cardinaux",
	journal =	"Fund. Math.",
	volume =	"3",
	year =		"1922",
	pages =		"1-6"
}

@article{sierpinski:leq,
	author =	"W. Sierpinski",
	title =		"Sur l'implication $2m\leq 2n \rightarrow m \leq n$ pour les nombres cardinaux",
	journal =	"Fund. Math.",
	volume =	"34",
	year =		"1947",
	pages =		"148-154"
}

@article{tarski:cancellation,
	author =	"A. Tarski",
	title =		"Cancellation laws in the arithmetic of cardinals",
	journal =	"Fundamenta Mathematica",
	volume =	"36",
	year =		"1949",
	pages =		"77-92"
}

